Integer Reset Timed Automata: Clock Reduction and Determinizability

In this paper, we propose a procedure that given an integer reset timed automaton (IRTA) ${\cal A}$, produces a language equivalent deterministic one clock IRTA ${\cal B}$ whose size is at most doubly exponential in the size of ${\cal A}$. We prove that this bound on the number of locations is tight. Further, if integer resets are used in stopwatch automata, a subclass of stopwatch automata which is closed under all boolean operations and for which reachability is decidable is obtained.

==> figs/comp_det_irta_combined.tex <==
\begin{figure} %TODO reduce the size of this graph
\begin{center}
\begin{picture}(50,35)(30,0)

\node[Nmarks=ir,iangle=180,ilength=3](S)(2,5){$\ \ \ \ s\ \ \ \ $}

\drawloop[loopdiam=4,loopangle=90](S){$\begin{array}{c}d_1,d_2,d_3\\d_4,d_5\end{array}$}  

\node[Nmarks=ir,iangle=180,ilength=2](S1)(20,25){$S1$}
\node[Nmarks=r](S2)(50,25){$S2$}
\node[Nmarks=r](S4)(80,25){$S4$}
\node[Nmarks=r](S5)(110,25){$S5$}
\node[Nmarks=r](S3)(50,5){$S3$}
\node[Nmarks=r](S6)(80,5){$S6$}
\node[Nmarks=r](S7)(110,5){$S7$}

\drawloop[loopdiam=4](S1){$\begin{array}{c}e1,c1\\a3\end{array}$}
\drawloop[loopdiam=4](S2){$b0,e1,a3$}
\drawloop[loopdiam=4,loopangle=270](S3){$e0,a2$}
\drawloop[loopdiam=4](S4){$b0,b1,e1,a3$}
\drawloop[loopdiam=4](S5){$e1,c1,a3$}
\drawloop[loopdiam=4,loopangle=270](S6){$e0,a2$}
% {$\begin{array}{c}e0\\a2\end{array}$}
\drawloop[loopdiam=4,loopangle=270](S7){$a0,a2$}
% {$\begin{array}{c}a0\\a2\end{array}$}

\drawedge[curvedepth=4](S1,S2){$b1$}

\drawedge[curvedepth=2,ELside=r](S2,S1){$c0$}
\drawedge[curvedepth=4,ELpos=50,ELside=l](S2,S3){$\begin{array}{c}e0\\a1\end{array}$}
\drawedge(S2,S4){$b1$}
\drawedge[curvedepth=14](S2,S5){$c1$}

\drawedge(S3,S1){$c0$}
\drawedge[curvedepth=4](S3,S2){$b0$}

\drawedge[ELside=r,ELpos=65](S4,S7){$a1$}
\drawedge[curvedepth=4,ELside=r](S4,S5){$c0,c1$}
\drawedge[curvedepth=4,ELside=r,ELpos=50](S4,S6){$e0$}

% \drawedge(S5,S7){$a1$}
% \drawqbpedge[sxo=-1,syo=-2,exo=2,eyo=-2,ELside=l,ELpos=70](S5,60,S3,165){$a1$}

\drawedge[curvedepth=4,ELside=r](S5,S4){$b1$}
\drawedge(S5,S7){$\begin{array}{c}a0\\a1\end{array}$}

\drawedge[curvedepth=4,ELside=l,ELpos=40](S6,S4){$b0$}
\drawedge[ELside=r,ELpos=30](S6,S5){$c0$}

\end{picture}
\end{center} 
 \caption{IRTA ${\cal A}$ and its deterministic IRTA ${\cal A}'$. The locations $S1$, $S2$, $S3$, $S4$, $S5$, $S6$ and $S7$ represent $\{S,0\}$, $\{(S,0),(S,1)\}$, 
$\{(S,1)\}$, $\{(S,0),(S,1),(S,1^+)\}$, $\{(S,0),(S,1^+)\}$, $\{(S,1),(S,1^+)\}$ and $\{(S,1^+)\}$ respectively. 
Here the symbols represent the following timed transitions $d_1::=b,x=1?,x:=0$, $d_2::= b, x \geq 1?$, $d_3::= c,x=1?x:=0$, $d_4::= c,x >1?$, $d_5::= e,x\geq 1?$, $b0::= b,n=0?$, $b1::= b,n=1?,n:=0$, $c0::= c,n=0?$, $c1::= c,n=1?,n:=0$, $e0::= e,n=0?$, $e1::= e,n=1?$, $a0::= b,n=0?; c,n=0?; e,n=0?$, $a1::= b,n\in(0,1)?; c,n\in(0,1)?; e,n\in(0,1)?$, $a2::= b,n>0?; c,n>0?; e,n>0?$ and $a3::= b,n>1?; c,n>1?; e,n>1?$.}
\label{fig_comp_det_irta}
\end{figure} 
\vspace*{-.5cm}
